Discovering Differences in the Representation of People using Contextualized Semantic Axes

A common paradigm for identifying semantic differences across social and temporal contexts is the use of static word embeddings and their distances. In particular, past work has compared embeddings against "semantic axes" that represent two opposing concepts. We extend this paradigm to BERT embeddings, and construct contextualized axes that mitigate the pitfall where antonyms have neighboring representations. We validate and demonstrate these axes on two people-centric datasets: occupations from Wikipedia, and multi-platform discussions in extremist, men's communities over fourteen years. In both studies, contextualized semantic axes can characterize differences among instances of the same word type. In the latter study, we show that references to women and the contexts around them have become more detestable over time.

==> alt_section_2.tex <==
\section{Constructing semantic axes}\label{sec:construct}

% static embeddings
Several formulae for calculating the similarity of a target word to two sets of pole words have been proposed in prior work on static semantic axes. These differ in whether they take the difference between a target word's similarities to each pole \cite{turney2003measuring}, calculate a target word's similarity to the difference between pole averages \cite{an-etal-2018-semaxis,kwak2021frameaxis}, or calculate a target word's similarity to the average of several word pair differences that represent the same antonymous relationship \cite{kozlowski2019geometry}. We build on the approach of \citet{an-etal-2018-semaxis} and \citet{kwak2021frameaxis}, because it does not require us to curate multiple paired antonyms for each axis, and it draws out the difference between two concepts before a target word is compared to them, rather than after. We define an axis $V$ containing antonymous sets of adjective vectors, $S_l = \{l_1, l_2, l_3, ..., l_n\}$ and $S_r= \{r_1, r_2, r_3, ..., r_m\}$, as the following: 
$$V = \frac{1}{n}\sum_{i=1}^n l_i - \frac{1}{m}\sum_{j=1}^m r_j.$$

Relying on single-word poles for axes can be unstable to the choice of each word \cite{an-etal-2018-semaxis,antoniak-mimno-2021-bad}. \citet{an-etal-2018-semaxis} creates a pole's set of words using the nearest neighbors of a seed word, which may risk conflating unintended meanings or antonymous neighbors \cite{mrksic-etal-2016-counter}. For example, one axis uses the opposite seed words \textit{green} and \textit{experienced}, but \textit{green}'s nearest neighbors include \textit{red} rather than \textit{inexperienced}. We construct poles using WordNet antonym relations, and each end aggregates synonymous and similar lemmas in WordNet synsets, which are expanded using the \textit{similar to} relation \cite{miller-1992-wordnet}.  We use this source to construct both static semantic axes (as in past work), and our contribution of contextualized semantic axes.

\paragraph{Static semantic axes.}
Our type-based embedding baseline, \textsc{glove}, uses 300-dimensional GloVe vectors pretrained on Wikipedia and Gigaword \cite{pennington-etal-2014-glove}. We only keep poles where both sides have at least three adjectives that appear in the GloVe vocabulary, and we also exclude acronyms, which are often more ambiguous in meaning. We start with 723 axes, where poles have on average 9.63 adjectives each. 

% BERT

\paragraph{Contextualized semantic axes.} Static embeddings, however, present a number of limitations.  Perhaps most importantly, such embeddings only allow for the orientation of a word \emph{type} on a semantic axis, effectively ignoring polysemy or homonymy \cite{wiedemann-etal-2019-does} and preventing analysis of token-based semantic variation (e.g., measuring whether a given mention of the word ``woman'' in context is depicted as more or less \textsc{beautiful} than another mention).  To enable this kind of analysis, we build contextualized semantic axes that use the same WordNet-based formulation as our GloVe baseline. Rather than each word in $S_l$ or $S_r$ being represented by a single GloVe embedding, we obtain BERT embeddings over multiple occurrences of each adjective. We use BERT-base, as this model is small enough for efficient application on large datasets and is popular in previous work on semantic change and differences \citep[e.g.][]{hu-etal-2019-diachronic, lucy-bamman-2021-characterizing,giulianelli-etal-2020-analysing,zhou-etal-2022-richer,coll-ardanuy-etal-2020-living,martinc-etal-2020-leveraging}. It is also used in tutorials for researchers outside of NLP, which means it has high potential use in computational social science and cultural analytics \cite{berthumanists2022}.

% BERT-prob
To build these contextualized axes, we obtain a potential pool of contexts for adjectives sampled over all of Wikipedia from December 21, 2021, preprocessed using \citet{Wikiextractor2015}'s text extractor. This sample contains up to 1000 sentences, or contexts, that contain each adjective, and we avoid contexts that are too short (over 10 tokens) or too long (over 150 tokens).\footnote{This length cutoff made the data more manageable, and 90\% of BERT's training steps were originally on 128-length sequences \cite{devlin-etal-2019-bert}.}

We experiment with two methods of obtaining contextualized BERT embeddings for each adjective: a random ``default"  (\textsc{bert-default}) and one where contexts are picked based on word probabilities (\textsc{bert-prob}). For \textsc{bert-default}, we take a random sample of 100 contextualized embeddings across the adjectives in each pole.  Since words can be nearest neighbors with their antonyms in semantic space \cite{mrksic-etal-2016-counter}, however, our main approach, \textsc{bert-prob}, aggregates word embeddings over contexts that highlight \emph{contrasting} meanings of axes' poles. 
To select contexts, we mask out the target adjective in each of its 1000 sentences, and have BERT-base predict the probabilities of synonyms and antonyms for that masked token. We remove contexts where the average probability of antonyms is greater than that of synonyms, sort by average synonym probability, and take the top 100 contexts. One limitation of our approach is that predictions are restricted to adjectives that can be represented by one wordpiece token. If none of the words on a pole of an axis appear in BERT's vocabulary, we backoff to \textsc{bert-default} to represent that axis.

%In later downstream analyses, we only keep poles that demonstrate separability between the two ends. 

For each of these BERT axes types, we also have versions where words' embeddings are $z$-scored, which has been shown to improve alignment with humans' word similarity judgements \cite{timkey-van-schijndel-2021-bark}. For $z$-scoring, we calculate mean and standard deviation embeddings from a sample of around 370k whole words from Wikipedia. As recommended by \citet{bommasani-etal-2020-interpreting}, we use mean pooling over wordpieces to produce word representations when necessary, and we extend this approach to create bigram representations as well. These embeddings are a concatenation of the last four layers of BERT, as these tend to capture more context-specific information \cite{ethayarajh-2019-contextual}. 
